Exploiting Vulnerabilities of Deep Learning-based Energy Theft Detection in AMI through Adversarial Attacks

Effective detection of energy theft can prevent revenue losses of utility companies and is also important for smart grid security. In recent years, enabled by the massive fine-grained smart meter data, deep learning (DL) approaches are becoming popular in the literature to detect energy theft in the advanced metering infrastructure (AMI). However, as neural networks are shown to be vulnerable to adversarial examples, the security of the DL models is of concern. In this work, we study the vulnerabilities of DL-based energy theft detection through adversarial attacks, including single-step attacks and iterative attacks. From the attacker's point of view, we design the \textit{SearchFromFree} framework that consists of 1) a randomly adversarial measurement initialization approach to maximize the stolen profit and 2) a step-size searching scheme to increase the performance of black-box iterative attacks. The evaluation based on three types of neural networks shows that the adversarial attacker can report extremely low consumption measurements to the utility without being detected by the DL models. We finally discuss the potential defense mechanisms against adversarial attacks in energy theft detection.

==> usefulInfo.tex <==
\cite{zheng2018novel} uses the attack model method, use the Irish dataset. use maximum information coefficient.

\cite{ismail2020deep} study the distributed generation domain, simulated dataset, detection rate 99.3\%, similar attack model method, combined deep neural network

\cite{zanetti2017tunable} define the attack model, use Irish dataset, use clustering method, around 84\% detection F1 score

\cite{gao2019physically} use linear regression, use the Southern California Edison (SCE) smart meter dataset, use the attack model, overall detection accu 80\%

\cite{nabil2018deep} use RNN, use Irish Dataset, use attack model, around 93\% accuracy


\cite{jokar2015electricity} use svm, use attack model, use Irish dataset, detection rate 94\%, false positive 11\%

\cite{punmiya2019energy} use svm, use attack model, use Irish dataset, around 95\% detection rate and 7\% false positive rate

\cite{zheng2017wide} uses CNN, use SGCC dataset.

\cite{hasan2019electricity} use CNN and LSTM

\cite{korba2018energy} use FNN, use Irish dataset




